BIOMEDICA: An Open Biomedical Image-Caption Archive, Dataset, and Vision-Language Models Derived from Scientific Literature

The development of vision-language models (VLMs) is driven by large-scale and diverse multimodal datasets. However, progress toward generalist biomedical VLMs is limited by the lack of annotated, publicly accessible datasets across biology and medicine. Existing efforts are restricted to narrow domains, missing the full diversity of biomedical knowledge encoded in scientific literature. To address this gap, we introduce BIOMEDICA, a scalable, open-source framework to extract, annotate, and serialize the entirety of the PubMed Central Open Access subset into an easy-to-use, publicly accessible dataset. Our framework produces a comprehensive archive with over 24 million unique image-text pairs from over 6 million articles. Metadata and expert-guided annotations are also provided. We demonstrate the utility and accessibility of our resource by releasing BMCA-CLIP, a suite of CLIP-style models continuously pre-trained on the BIOMEDICA dataset via streaming, eliminating the need to download 27 TB of data locally. On average, our models achieve state-of-the-art performance across 40 tasks - spanning pathology, radiology, ophthalmology, dermatology, surgery, molecular biology, parasitology, and cell biology - excelling in zero-shot classification with a 6.56% average improvement (as high as 29.8% and 17.5% in dermatology and ophthalmology, respectively), and stronger image-text retrieval, all while using 10x less compute. To foster reproducibility and collaboration, we release our codebase and dataset for the broader research community.

==> Figures/pull_figure.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{images/datamap.jpg}
    \caption{Comparison of the span of previous openly available biomedical datasets compared to \dataset\ \JN{Consider using the DataShader package for plots with \>500K points} }
    \label{fig:comparison}
\end{figure}

==> tables/local_for_global_taxonomy.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{lc}
\toprule
\rowcolor{gray!10} \textbf{Global Concept} & \textbf{Local Concept Count} \\
Chemical Structures & 7 \\
Clinical Imaging & 34 \\
Graph and Network & 2 \\
Hand Drawn and Screen Based Visuals & 11 \\
Illustrative Diagrams & 15 \\
Immuno Assays & 8 \\
Maps & 1 \\
Microscopy & 23 \\
Plots and Charts & 96 \\
Scientific Formulae and Equations & 1 \\
Tables & 2 \\
Tools and Materials & 3 \\
\bottomrule
\end{tabular}
\caption{Number of Local Concepts by Global Concepts}
\label{tab:local_class_counts}
\end{table*}


==> tables/metadata_list.tex <==
% ### Article
% - PMCID
% - PMID
% - Title
% - Abstract
% - Journal
% - Citation
% - License
% - Keywords
% - MeSH terms
% - Published Date (unix string)
% - Full text article (nXML)
% - Articles citing this paper list
% - Count of articles citing this paper list
% - Article category
% ### Image
% - Image hash
% - Image ID
% - Path to original image file
% - Figure Reference
% - Caption


% Share
% You said:
% All data and  metadata for each article is stored in JSON files Table \ref{} lits all data extracted and porvdenace. 
% ChatGPT said:
% It seems you want to reference a table listing extracted data and provenance details for each article. Here’s a corrected version of your sentence:

% "All data and metadata for each article are stored in JSON files. Table \ref{} lists all the extracted data along with its provenance."

% Make sure to replace \ref{} with the appropriate reference label for your table.











